Transferable Cross-Chain Options

An option is a financial agreement between two parties to trade two assets. One party is given the right, but not the obligation, to complete the swap before a specified termination time. In todays financial markets, an option is considered an asset which can itself be transferred: while an option is active, one party can sell its rights (or obligations) to another. Todays blockchains support simple options in the form of cross-chain atomic swap protocols where one party has the choice whether to complete the swap. The options implemented by these cross-chain protocols, are not, however, transferable. This paper proposes novel distributed protocols for transferable cross-chain options, where both option owners and providers can sell their positions to third parties. The protocol ensures that none of the parties can be cheated, that no unauthorized party can interfere, and that the transfer succeeds if the buyer and seller faithfully follow the protocol.

==> future_work.tex <==
The described protocol is a first step towards devising more general protocols for transferring financial positions.
The key insight is that if an agent has various rights and obligations, then that agent's financial position itself is an asset to be traded. 

There are many natural ways our simple protocol can be extended.
For example, Alice might want to offer multiple candidates the opportunity to buy her position in the \textit{2-party swap} instead of just offering it to Carol.
This way, she can give herself more opportunities to interact with an honest counterparty and potentially receive a higher compensation for her swap position.
How she chooses the party that ultimately takes her position is also interesting in its own right.
She could for example run a \textit{second-price auction} whose winner takes her position.
The inevitable difficulty with such a setup of course, is designing a protocol that behaves correctly under the presence of dishonest coalitions and concurrent contract executions.
Additionally, Alice and Bob both might want to have the ability to transfer their position's concurrently.
This is the subject of future work.





Meeting notes:

If Bob calles mutatelock first, and it does not allow contest again, Carol still needs to wait for 2 delta.this seetting needs to be considered again.(Resolved. carol does not need to wait anymore)

It may be problematic if the timeout on AB and BA edge for mutatelOck is offset by 1 delta, since if Alice cheats, Bob cannot relay it to another chain in time, assume Bob has one more time than Alice to call mutate lock;(resolved. no offset)

The latest time to call mutate lock is $T - 7\Delta$. (leader protocol)

$T$ is timeout of $BA$.

Meeting accomplished:
for case of David replaces BOb, the timout for both mutatalock/attest called by BOb is $T-2\delta$;
For DB edged, the timeout is $now+4\delta$.

Friday meeeting:

Daniel:
Adjust last chance to mutate for Alice to be $T - 7\Delta$, Bob has one more delta than alice to mutate.
Change timeout for $CA$ edge to be $nw+8\Delta$.
Make sure revert function is consistent with new timeouts.


==> garbage.tex <==
\begin{comment}


\begin{property}
No underwater for conforming Alice.
\end{property}

\begin{proof}
Alice should own the option if she cannot get CA edge. If Alice gets CA edge, no matter what the graph is now, including partial ABSwap leftovers and partial  CBSwap established, she does not care. Thus, here we show that a conforming Alice's state satisfy the following predicate:

CA edge is triggered(case1) || Alice owns the ABSwap (case2)

\begin{enumerate}
    \item If Carol does not create CA edge, ABSwap does not change.
    \item If Carol creates CA edge, conforming Alice locks AB and BA edge and wait for Carol to exercise CASwap or not. 
    \begin{itemize}
        \item If Carol releases $C_1$ on both AB and BA edge, Alice can trigger CA edge.(case 1)
        \item If Carol releases $C_1$ on only one of AB and BA edge, Alice can trigger CA edge.(case 1)
        \item If Carol does not release $C_1$ at all, then after $R+3\Delta$, Alice gets back the ABSwap since it is unlocked by revert().(case 2)
    \end{itemize}
\end{enumerate}
Then, if Alice owns ABSwap, she either gets her asset refunded or loses her asset with Bob's asset. If Alice no longer owns total ABSwap, she must gets Carol's asset. Then, she either trade her asset with Carol's asset or get Carol's asset for free, either case is fine for her.
\end{proof}

\begin{property}
No underwater for conforming Carol.
\end{property}
\begin{proof}
For a conforming Carol, if she loses her CA edge, she must have CBSwap. Otherwise, she should get her asset on CA edge back.

 Thus, here we show that a conforming Carol's state satisfy the following predicate:

CA edge is refunded(case1) || Carol owns the CBSwap (case2)


A conforming Carol creates CA edge and only releases $c_1$ if Alice mutates both BA and AB edge with Carol's secret $c_1$ and $c_2$. After Alice mutates BA and AB, she also wait until there is no possible contest to break the tentative transfer from ABSwap to CBSwap. Since Carol only releases $c_1$ after she confirms that releasing it would change ABSwap to CBSwap, if she releases $c_1$ and loses CA edge, she gets  CBSwap(case2). Otherwise, she keeps her secret and then CA edge is refunded after timeout.


Then, if Carol has CBSwap, she can exercise her option to get Bob's asset, with/without losing her CA edge, where either is fine. She can also choose not to exercise her option, getting Alice's asset, with/without losing her CA edge, where either is fine.

If Carol does not own CBSwap, by the predicate we show, her asset is refunded, which is also fine for Carol.
\end{proof}

\begin{property}
No underwater for Bob.
\end{property}

\begin{proof}

Here, Bob is selling an optionality to someone. He does not care who the trader is, as long as he can guarantee that when he loses his asset previously escrowed on BA edge, he can get the asset previously escrowed on AB edge.

Thus, Bob needs to guarantee that, no matter what edge his asset is on, the secret to trigger it is the same as that of his incoming edge.

We start from ABSwap and show that any modification on AB edge will be reflected on BA edge within $\Delta$ after AB's modification and vice versa. In $2\Delta$ , two edges are synchronized.

First we show any state update on AB edge will show up on BA edge within $\Delta$.

On AB edge, first it is locked by $s_a$ and it is ready to be claimed as long as $s_a$ by timeout. We define  the state  as $READY2CLAIM(s_a)$. In the period of transferring the option, the contract state can be $LOCKED(C_1,s)$  meaning no one can claim the asset and $C_1$ is needed to release the lock or by timeout.  After it is unlocked, the state is updated to $READY2CLAIM(s)$ which can be claimed by some $s$. If the contract is claimed by $s$, the state is denoted as $CLAIMED(s)$. If the contract is expired, the state is denoted as $REFUNDED$.


AB edge is initialized as $READY2CLAIM(s_a)$. Then, if AB edge is updated to $LOCKED(C_1,s)$ state, then within $\Delta$, Bob can send Alice's mutation to $BA$ edge. In the same time, $BA$ edge can be in $READY2CLAIM(s_a)$ or $LOCKED(C_1,s)$ or $CLAIMED(s_a)$ state. 
\begin{enumerate}
    \item If $BA$ edge  is in $READY2CLAIM(s_a)$, then Bob updates it to $LOCKED(C_1,s)$ state.
    \item If BA edge is in $LOCKED(C_1',s')$ state where either $C_1'\neq C_1$ or $s'\neq s$, then Bob contests it with $LOCKED(C_1,s)$ on BA edge and turns the BA edge to  $READY2CLAIM(s_a)$ state.  In the meantime, Bob sends the mutation of $LOCKED(C_1',s')$ signed by Alice to AB edge and make AB edge back to $READY2CLAIM(s_a)$ state. It takes $2\Delta$ to synchronize two edges.
    \item  If $BA$ edge is in $CLAIMED(s_a)$ state, then Bob can send Alice's secret $s_a$ to edge $AB$ to claim AB edge by contesting  $LOCKED(C_1,s)$. Then both AB and BA edge is in the $CLAIMED(s_a)$ state.

\end{enumerate}


AB edge is updated from $LOCKED(C_1,s)$ to  $READY2CLAIM(c_2)$ state by Carol only if Bob approves it or Bob does not contest. That means, an honest Bob observes two edges are in the same $LOCKED(C_1,s)$ state. Otherwise, he contests and turn the states of both edges to either case (2) or case(3) . If there is no contest, Carol sends $c_1$ to the pending mutation to replace Alice's role, move it to $READY2CLAIM(c_2)$. Then within $\Delta$, Bob can send Carol's secret to $BA$ edge and make BA edge $READY2CLAIM(c_2)$.  When Bob sends Carol's secret to BA edge, the only possible state on BA edge is $LOCKED(C_1,s)$ or $READY2CLAIM(c_2)$ since two edges are synchronized before $READY2CLAIM(c_2)$ is possible.

The rest is the same as an atomic swap CBSwap.

It is also possible that AB edge is updated from $LOCKED(C_1,s)$ back to $READY2CLAIM(s_a)$ because Carol does not release $c_1$. Suppose Alice's mutation happens at time $t$. $READY2CLAIM(s_a)$  happens at $t+4\Delta$. If BA edge is in $LOCKED(C_1,s)$, it must happens within $t+\Delta$. Then in $t+5\Delta$, BA edge is back to $READY2CLAIM(s_a)$. During $t+4\Delta$ to $t+5\Delta$, Carol cannot release $c_1$ to change BA edge from $LOCKED(C_1,s)$ to $READY2CLAIM(s)$ due to the timeout.

Thus, $BA$ edge is guaranteed to revert to $READY2CLAIM(s_a)$.

The synchronization between BA edge and AB edge are mostly symmetric, except that when Bob sends a mutation from BA edge to AB edge, if AB edge is in $CLAIMED(s_a)$ state, Bob is fine from now since he gets Bob's asset for free or in exchange. 


\end{proof}

To show that no conforming party is underwater, we will show that if, a party is conforming to the reselling protocol, then it is equivalent to their view that they are setting up CASwap to try to exchange ABSwap to CBSwap.

First, here is the reselling protocol.

STEP 1: Alice puts $mutate(c_1,c_2)$ on both AB and BA edge;

STEP 2: Carol sends $c_1$ to both AB and BA edge until no contest is possible.


\begin{enumerate}
    \item No underwater for Alice. If Alice is conforming, she locks both edges, and Bob cannot contest. Then it is equivalent that she escrowed ABSwap to Carol on CA edge by $R+3\Delta$ , with timeout $R+5\Delta$ assuming Carol creates CA by $R$. Then, (1)if Carol exercises CASwap and conforming to the reselling protocol and ABSwap is changed to CBSwap. (2) if Carol exercises  CASwap and is not conforming to the reselling protocol, Alice gives up ABSwap and in exchange gets assets on CA edge.
    (3) if Carol does not exercise her swap, Alice gets her ABSwap back.
    
    \item No underwater for Carol. If Carol is involved in CASwap. She first creates CA edge and waiting for Alice to escrow her ABSwap. If and only if both edges of ABSwap are locked and no longer be able to be contested, it is really count as escrowed. Then from Carol's view, if she is conforming to the reselling protocol, then:(1) if she exercises CASwap, she will turn ABSwap to CBSwap; (2) if she does not exercise CASwap, her CA edge is refunded.
    
    \item No underwater for Bob. We will show that if Bob is conforming to reselling protocol(reporting inconsistent change), then from the perspective of Bob, ABSwap is either never escrowed in CASwap or ABSwap is escrowed and triggering CA edge has the effect of turning ABSwap to CBSwap.
    
   If Alice is conforming in reselling protocol, then ABSwap is escrowed. And if Carol is conforming in reselling protocol, then ABSwap turns into CBSwap. If Alice is not conforming in reselling protocol, then by $R+3\Delta$, ABSwap cannot be escrowed on AC edge, since Bob would reverted locked edges to the normal ABSwap. From Bob's view, ABSwap preserves. If Alice is conforming and ABSwap is escrowed, and then if Carol is not conforming, a conforming Bob can create a view the same as that where Carol is conforming. That being said, if Carol is not conforming by releasing her secret only on one edge, then because of the different timeout set by different parties, Bob always have one more round to send Carol's secret to another edge. Thus, the two edges either both receive $c_1$ by $R+5\Delta$ or none of them receive  $c_1$. This is exactly what would be if Carol is conforming. Thus we complete the proof.
\end{enumerate}
\end{comment}
